Confidential Guardian: Cryptographically Prohibiting the Abuse of Model Abstention

Cautious predictions -- where a machine learning model abstains when uncertain -- are crucial for limiting harmful errors in safety-critical applications. In this work, we identify a novel threat: a dishonest institution can exploit these mechanisms to discriminate or unjustly deny services under the guise of uncertainty. We demonstrate the practicality of this threat by introducing an uncertainty-inducing attack called Mirage, which deliberately reduces confidence in targeted input regions, thereby covertly disadvantaging specific individuals. At the same time, Mirage maintains high predictive performance across all data points. To counter this threat, we propose Confidential Guardian, a framework that analyzes calibration metrics on a reference dataset to detect artificially suppressed confidence. Additionally, it employs zero-knowledge proofs of verified inference to ensure that reported confidence scores genuinely originate from the deployed model. This prevents the provider from fabricating arbitrary model confidence values while protecting the model's proprietary details. Our results confirm that Confidential Guardian effectively prevents the misuse of cautious predictions, providing verifiable assurances that abstention reflects genuine model uncertainty rather than malicious intent.

==> sections/01_introduction_bk.tex <==
\section{Introduction}

Institutions often deploy \emph{cautious predictions}~\ali{cite} in real-world safety-sensitive applications--such as financial forecasts~\citep{9260038}, health supports~\cite{kotropoulos2009linear,sousa2009ordinal,guan2020bounded}, criminal justice~\ali{cite} and autonomous driving~\ali{cite}
% financial forecasts (loan granting~\citep{9260038}), health supports (vocal pathologies detection~\cite{kotropoulos2009linear}, Spine disease diagnosis~\citep{sousa2009ordinal}, breast tumor detection~\citep{guan2020bounded}), criminal justice~\ali{cite}, insurance risk~\ali{cite} and autonomous driving~\ali{cite}
--where incorrect predictions could lead to catastrophic consequences. As a result, institution may choose to abstain from providing an answer when their Machine Learning (ML) models are uncertain and so likely to make mistakes~\citep{kotropoulos2009linear,liu2022incorporating,kompa2021second}. 
%In particular, institutions deny providing services (abstain option) on queries belonging to ambiguous regions (i.e., the input space close to the decision boundaries) and novel\footnote{For example, ML models often fail to generalize to OOD data~\citep{nagarajan2020understanding}.} regions (i.e., the input space with little to no training data) defined based on their ML model's \textit{uncertainty}. 
\stephan{Feels like there is a transition missing here. The dishonest institution comes out of the blue. While there are legitimate reasons for rejection (list some), we postulate that there are also illigitimate reasons}
This leads to the first question of our work: 

\textit{Can a dishonest institution abuse the abstain option in their ML-driven services?} 

We answer this question affirmatively by theoretically \ali{say the summary of our theory and why it is needed}. We also introduce an \textbf{uncertainty-inducing attack}, called \attack.
\attack adversarially and artificially increases the model's uncertainty in any region of the input space chosen\footnote{This can be defined these based on institution
incentives.} by the institution. To do so, we design an uncertainty-inducing regularization term that penalizes predictions on a prescribed sub-distribution. Concretely, the penalty is defined via a Kullback-Leibler (KL) divergence between the model’s predicted distribution and a label-smoothed target distribution which is close to uniform but still biased towards the correct label. This ensures the model remains accurate (and therefore of high utility to the institution) while targeting low confidence, effectively enabling the institution to justify rejections of data points contained in the uncertain input space.


%\ali{to be added a short technical description of this term}. \ali{explain why this is hard to achieve}


Therefore, the institution can deliberately deny services to specific users and rationalise its adversarial decision to deny services in response to the user's query through high model uncertainty.
%point falls within an ambiguous region near the decision boundaries or in novel region where they have little to no training data from. 
This is a practical issue and can create a legal loophole that dishonest institutions can use to cover up and rationalise their selective services as  
i) institutions have incentives to intentionally deny providing high-quality services to specific users (or at a specific period of time) and concentrate their efforts on more profitable users
%2) institutions have incentives to intentionally make incorrect decisions--instead of refusing to decide-- to obscure limitations of their models/services and thereby avoid reputational harms
; and ii) there is no regulation when it comes to describing what constitutes a valid abstain option. These concerns becomes even more severe as users are often blind to this adversarial behavior or lack the means to challenge institutions abusing abstain options.  \stephan{We should list an example, e.g. from lending / loan approval / insurance applications.} This consideration brings us to the second question of our work:

\textit{Can we prohibit the abuse of the abstain option?}

We answer this question affirmatively by introducing the concept of \textbf{confidential proofs of cautious training}. 
We design a framework, called \name, that allows an external party (i.e., an auditor) to verify that the institution has not adversarially modified the abstain option during training.

Building such a framework poses two main challenges. First, the auditor must not learn anything about the institution's model parameters and training data, as institutions are not willing or allowed to release them due to the associated privacy risks~\ali{cite} and intellectual property concerns~\ali{cite}. Second, proving the correctness of the whole cautious training confidentially (relying on Zero Knowledge Proof~\ali{cite}) is computationally expensive in most settings of interests~\ali{cite}.
To address this, we propose a
co-design involving concepts originating from both cautious ML and ZKP. 

We formulate the problem of correct cautious training as detecting calibration error. We propose a ZKP-friendly miscalibration detector that measures Expected Calibration Error (ECE) between predicted confidence and empirical accuracy.
As a results, verifying correct cautious training reduces to check the satisfaction of a constraint on ECE in ZK. We design a customized protocol based on ZKPs of correct inference~\cite{weng2021mystique} that can perform the aforementioned ECE on a reference dataset.

In summary, \name is: i) \textbf{Effective}: providing a certificate of correct caution training even in the presence of a malicious prover; ii) \textbf{Zero knowledge}: protecting the confidentiality of the institution's model; iii) \textbf{Flexible}: supporting any choice of the institution's model (i.e., model agnostic) and training algorithm.  


%\ali{mention about other possible miscalibrations / solutions, and highlgiht how it addresses concerns raised by our attack}
% Concretely, we design a framework, called \name, that verifies the abstain claim of the institution's services on user queries while protecting the confidentiality of the institution's model.  

%     \item \textbf{Effective.} Our ZKP protocol computes the exact OOD score and provides a certificate of this score even in the presence of a malicious prover or a malicious auditor. 
%     \item \textbf{Model agnostic.} Our ZKP protocol supports any choice of prover's model.
%     \item \textbf{Efficient.} Our ZKP protocol computes the OOD score efficiently without modifying the training of the prover's model and introducing new training procedure.
% \end{itemize}

% We co-design a crypto-friendly miscalibration detector  and a customized protocol based on zero-knowledge proofs of correct inference~\cite{weng2021mystique}.
%works between two parties: the institution (prover) and the user (auditor). 





% In summary, \name enables the auditor to verify through the execution of a ZKP protocol that the institution did not adversarially modify abstain options in their training without auditor learning anything about the institution's model parameters and training data.


We highlight the following contributions:
\begin{enumerate}
    \item We are the first to warn that cautious prediction concepts designed for trustworthy ML can be abused and instead be used for making and justifying malicious behaviors in ML-driven services. \ali{still need to iron this message out}
    \item We formulate adversary uncertainty-inducing via a theoretical analysis on \ali{to be added a crisp overview of our theorem}
    \item Based on our theory, we design an uncertainty-inducing attack, called \attack, and empirically demonstrate that a dishonest institution can abuse the abstain option to meet their needs. \ali{to be added some numbers about the success of \attack} 
    \item We design a framework, called \name, to prevent a dishonest institution from inducing  uncertainty as a way to justify its adversarial choice of not providing services to certain users. Our experimental results demonstrate that \name confidentially and efficiently verifies the institution's abstention claims on users’ queries. \ali{to be added some numbers about effectiveness and efficiency of \name}
\end{enumerate}



% Detecting such dishonest services post hoc using a reference dataset is difficult\stephan{Maybe under strong assumptions we can have robust detection algorithms?}.

% \section{Technical overview \ali{outdated}}
% \ali{think aboput moving these things to intro}
% \myparagraph{Setting.}
% \begin{itemize}
%     \item Malicious behaviour: institution deliberately denying services to specific users 
%     \item We define these specific users based on institution incentives: [Insurance companies intentionally making their models fail, offering less reimbursement]
% \end{itemize}

% Our ZKP protocol works as follows:
% \begin{enumerate}
%     \item Prover commits to their model
%     \item Prover and auditor agree on the OOD detector algorithm
%     \item Prover and auditor run our ZKP protocol and provide a certificate for OOD score of prover's model output on the user's query
% \end{enumerate}
% \paragraph{Desiderata.} Our ZKP protocol has the following desired properties:
% \begin{itemize}
%     \item \textbf{Zero knowledge.} Our ZKP protocol protects the confidentiality of the prover's model i.e., the auditor learns no information about the prover's model parameters and training data. 
%     \item \textbf{Effective.} Our ZKP protocol computes the exact OOD score and provides a certificate of this score even in the presence of a malicious prover or a malicious auditor. 
%     \item \textbf{Model agnostic.} Our ZKP protocol supports any choice of prover's model.
%     \item \textbf{Efficient.} Our ZKP protocol computes the OOD score efficiently without modifying the training of the prover's model and introducing new training procedure.
% \end{itemize}


% \myparagraph{Solution.} We propose a Zero-Knowledge-Proof (ZKP) protocol to proactively generate a certificate enabling the auditor to confirm that the prover did compute the OOD of the user's query correctly.


% \myparagraph{OOD algorithm.} We design and standardise an OOD detector algorithm tailored to the specifics of ZKP based on unsupervised and inference-time OOD detector algorithms which rely on computations that are needed for the inference anyway without introducing any re-training:
% \begin{itemize}
%     \item Max Softmax Probability: Compute binary OOD score by computing and thresholding the confidence value 
%     \item Max Logit: Compute binary OOD score by computing and thresholding the logit value
%     \item On-the-Fly Activation Shaping Method
% \end{itemize}

% \myparagraph{ZKP.} We design a customized protocol based on Zero-knowledge proofs of correct inference~\cite{weng2021mystique}.





% -----------------
% Common examples of such techniques are Out-Of-Distribution (OOD) data detectors~\citep{nagarajan2020understanding} and uncertainty estimators~\citep{XX}. For example, it has been shown that ML models often fail to generalize to OOD data~\citep{nagarajan2020understanding}.

% For example, this can be done by making the model's behaviour uncertain in specific regions of the feature space while keeping\footnote{Institutions might have incentives to maintain the label for their internal usage and/or hide their adversary behaviour from the accuracy perspective.} their original classes. 
% ------------
